Non-Mergeable Sketching for Cardinality Estimation

Cardinality estimation is perhaps the simplest non-trivial statistical problem that can be solved via sketching. Industrially-deployed sketches like HyperLogLog, MinHash, and PCSA are mergeable, which means that large data sets can be sketched in a distributed environment, and then merged into a single sketch of the whole data set. In the last decade a variety of sketches have been developed that are non-mergeable, but attractive for other reasons. They are simpler, their cardinality estimates are strictly unbiased, and they have substantially lower variance. We evaluate sketching schemes on a reasonably level playing field, in terms of their memory-variance product (MVP). E.g., a sketch that occupies $5m$ bits and whose relative variance is $2/m$ (standard error $\sqrt{2/m}$) has an MVP of $10$. Our contributions are as follows. Cohen and Ting independently discovered what we call the Martingale transform for converting a mergeable sketch into a non-mergeable sketch. We present a simpler way to analyze the limiting MVP of Martingale-type sketches. We prove that the \Martingale{} transform is optimal in the non-mergeable world, and that \Martingale{} \fishmonger{} in particular is optimal among linearizable sketches, with an MVP of $H_0/2 \approx 1.63$. E.g., this is circumstantial evidence that to achieve 1\% standard error, we cannot do better than a 2 kilobyte sketch. \Martingale{} \fishmonger{} is neither simple nor practical. We develop a new mergeable sketch called \Curtain{} that strikes a nice balance between simplicity and efficiency, and prove that \Martingale{} \Curtain{} has limiting $\MVP\approx 2.31$. It can be updated with $O(1)$ memory accesses and it has lower empirical variance than \Martingale{} \LogLog, a practical non-mergeable version of HyperLogLog.

==> backup.tex <==

\begin{theorem}\label{thm:me}
(Ting also got equivalent results for $\E(E_\lambda)$ and $\Var(E_\lambda)$ from another perspective (using Doob's decomposition, for area cutting processes with offset decompositions), but he said that $V_k$ is inadequate for estimating the variance at a fixed $\lambda$ and one needed to take Bayesian argument to compensate the $(n-T_K)$ part. This theorem uses a more elementary proof and says $V_k$ \emph{is} an unbiased estimation of the variance.)
\begin{align*}
    \E(E_\lambda) =\lambda,\text{ and } \Var (E_\lambda)=\E(V_\lambda) = \sum_{k=1}^\lambda 
    \E\paren{\frac{1}{P_k}}-\lambda.
\end{align*}
\end{theorem}
\begin{proof}
Note that $P_k$ is a function of $S_{k-1}$. 
By the linearity of expectation and the law of total expectation, we have
\begin{align*}
    \E(E_\lambda) &= \sum_{k=1}^\lambda \E\left(\mathbbm{1}[S_k\neq S_{k-1}]\frac{1}{P_k}\right)
    = \sum_{k=1}^\lambda \E\left(\E\left(\mathbbm{1}[S_k\neq S_{k-1}]\frac{1}{P_k}\mid S_{k-1}\right)\right)\\
    &= \sum_{k=1}^\lambda \E\left(\E\left(\mathbbm{1}[S_k\neq S_{k-1}]\mid S_{k-1}\right)\frac{1}{P_k}\right)\\
    &= \sum_{k=1}^\lambda \E\left(\Pr(S_k\neq S_{k-1}\mid S_{k-1})\frac{1}{P_k}\right)
    =\sum_{k=1}^\lambda \E(1)
    = \lambda,
\intertext{and} 
    \E(V_\lambda) &= \sum_{k=1}^\lambda \E\left(\mathbbm{1}[S_k\neq S_{k-1}]\frac{1-P_k}{P_k^2}\right)\\    &= \sum_{k=1}^\lambda \E\left(\E\left(\mathbbm{1}[S_k\neq S_{k-1}]\mid S_{k-1}\right)\frac{1-P_k}{P_k^2}\right)\\
    &= \sum_{k=1}^\lambda \E\left(\frac{1-P_k}{P_k}\right)
    = \sum_{k=1}^\lambda \E \paren{\frac{1}{P_k}}-\lambda,
\end{align*}
For the variance,  we have
\begin{align*}
    \Var(E_\lambda) =& \E(E_\lambda^2)-(\E(E_\lambda))^2\\
    &= \E\left(\sum_{k=1}^\lambda \mathbbm{1}[S_k\neq S_{k-1}]^2\frac{1}{P_k^2}+2\sum_{r<k}\mathbbm{1}[S_k\neq S_{k-1}]\cdot \mathbbm{1}[S_r\neq S_{r-1}]\cdot \frac{1}{P_kP_r} \right)-\lambda^2.
\end{align*}

We first calculate that
\begin{align*}
    \E\left(\mathbbm{1}[S_k\neq S_{k-1}]^2\cdot \frac{1}{P_k^2}\right)=\E\left(\E\left(\mathbbm{1}[S_k\neq S_{k-1}]^2 \;\middle|\; S_{k-1}\right)\frac{1}{P_k^2}\right)=\E\paren{\frac{1}{P_k}}.
\end{align*}

Then note that for any $r<k$, by the law of total expectation, we have
\begin{align*}
    \lefteqn{\E\left(\mathbbm{1}[S_k\neq S_{k-1}]\cdot \mathbbm{1}[S_r\neq S_{r-1}]\cdot \frac{1}{P_kP_r}\right)}\\
    &=\E\left(\E\left(\mathbbm{1}[S_k\neq S_{k-1}]\cdot \mathbbm{1}[S_r\neq S_{r-1}]\cdot \frac{1}{P_k} \;\middle|\; S_{r-1}\right) \frac{1}{P_r} \right)\\
    &=\E\left(\E\left(\mathbbm{1}[S_k\neq S_{k-1}]\cdot \frac{1}{P_k} \;\middle|\; S_r\neq S_{r-1}, S_{r-1}\right)\Pr(S_r\neq S_{r-1}, S_{r-1}) \frac{1}{P_r} \right)\\
    &=\E\left(\E\left(\mathbbm{1}[S_k\neq S_{k-1}]\cdot \frac{1}{P_k} \;\middle|\; S_r\neq S_{r-1},  S_{r-1}\right)\right)
\end{align*}

Let $s\in\mathcal{S}$. 
Conditioning on $S_{r-1}=s$, since $r\leq k-1$, we have
\begin{align*}
    \Pr(S_r\neq s,S_{r-1}=s)=\sum_{s_1,\ldots,s_{k-1}}\mathbbm{1}[s_r\neq s, s_{r-1}=s]\Pr(S_1=s_1,\ldots,S_{k-1}=s_{k-1}).
\end{align*}

Thus we have
\begin{align*}
    \lefteqn{\E\left(\mathbbm{1}[S_k\neq S_{k-1}]\cdot \frac{1}{P_k} \;\middle|\; S_r\neq s, S_{r-1}=s\right)}\\
    &=\frac{\displaystyle\sum_{s_1,\ldots,s_{k-1}}\mathbbm{1}[s_r\neq s, s_{r-1}=s]\Pr(S_1=s_1,\ldots,S_{k-1}=s_{k-1})\E\left(\mathbbm{1}[S_k\neq S_{k-1}]\frac{1}{P_k}\mid S_1=s_1,\ldots,S_{k-1}=s_{k-1} \right)}{\displaystyle \sum_{s_1,\ldots,s_{k-1}}\mathbbm{1}[s_r\neq s, s_{r-1}=s]\Pr(S_1=s_1,\ldots,S_{k-1}=s_{k-1})}\\
    &=1,
\end{align*}
since 
\begin{align*}
    \lefteqn{\E\left(\mathbbm{1}[S_k\neq S_{k-1}]\cdot \frac{1}{P_k} \;\middle|\; S_1=s_1,\ldots,S_{k-1}=s_{k-1} \right)}\\
    &=\E\left(\frac{\mathbbm{1}[S_k\neq S_{k-1}]}{\Pr(S_k\neq S_{k-1}\mid S_{k-1})} \;\middle|\; S_1=s_1,\ldots,S_{k-1}=s_{k-1} \right)\\
    &=\frac{\E(\mathbbm{1}[S_k\neq S_{k-1}]\mid S_{k-1}=s_{k-1})}{\Pr(S_k\neq S_{k-1}\mid S_{k-1}=s_{k-1})}=1.
\end{align*}

Thus we have
\begin{align*}
    \lefteqn{\E\left(\mathbbm{1}[S_k\neq S_{k-1}]\cdot \mathbbm{1}[S_r\neq S_{r-1}]\cdot \frac{1}{P_kP_r}\right)}\\
    &=\E\left(\E\left(\mathbbm{1}[S_k\neq S_{k-1}]\cdot \frac{1}{P_k}\;\middle|\; S_r\neq S_{r-1}, S_{r-1}\right)\right)=\E(1)=1.
\end{align*}

Finally, by the linearity of expectation we have
\begin{align*}
    \Var(E_\lambda)= \sum_{k=1}^\lambda \E \paren{\frac{1}{P_k}} +2\frac{\lambda(\lambda-1)}{2}\cdot 1 - \lambda^2=\sum_{k=1}^\lambda \E \paren{\frac{1}{P_k}}-\lambda 
    = \E(V_\lambda).
\end{align*}
\end{proof}

==> backup2.tex <==
\section*{Backup}
In this section, we will establish the framework of defining and analyzing sketches as a well-behaved abstract model. We start from rephrasing the sketches' original definitions using the language of random variables. Then we introduce the asymptotic approximation and the smoothing technique. These steps bring us abstract definitions of practical sketches which are strictly scale-invariant (Definition \ref{def:scale-invariant}) and coincides with the behavior of their original definitions asymptotically.

We use $\qLL$ and $\qPCSA$ as examples to show how a sketch should be defined and analyzed in our framework. 
\subsection{Defining Sketches}
\subsubsection{Original Definitions}
For easier understanding, instead of introducing the sketches directly, we introduce a hierarchical view of how the sketches are derived. After $\lambda$ distinct insertions, the ``raw data'' the algorithm receives is $X(\lambda)=\{U^{(i)}\}_{i=1,\ldots,\lambda}$, where $U^{(i)}$s are \iid uniform random variable in $[0,1]$. The $\MIN$ sketch just stores the minimum of the hash values, i.e., $\min X(\lambda)$. It is inefficient in space to directly store the statistic in ``raw data'' and one often needs to quantize the interval $[0,1]$. A base-$q$ quantization of $X(\lambda)$ is a set of random variables $Y(q,\lambda)=\{Y_i(\lambda,q)\}_{i\geq 0}$, where for any $i\geq 0$,
\begin{align*}
    Y_i(\lambda,q)= \mathbbm{1}\left[ X(\lambda )\cap (\frac{1}{q^{i+1}},\frac{1}{q^{i}}]\neq \emptyset \right].
\end{align*}
It is straight forward to show that
\begin{align*}
    \Pr(Y_i(\lambda,q)=0)=(1-(\frac{1}{q^i}-\frac{1}{q^{i+1}}))^\lambda.
\end{align*}

(a diagram here?)
We can easily define many sketches as a base-$q$ quantization with a mask. Let $Z_i(\lambda)$
The $\qPCSA$ sketch is just the base-$q$ quantization $Y(q,\lambda)$ and the $\qLL$ sketch is the largest index of $1$, i.e., $\max \{ i \mid Y_i(\lambda,q)=1\}$. The state changing probabilities of these two sketches can be formally defined as follows.

\begin{definition}
Let the state changing probabilities of a sketch $A$ of the $\lambda$th insertion be denoted as $P_\lambda(A)$. Then we define:
\begin{align*}
    P_\lambda(\qPCSA)=&\sum_{i=0}^\infty Y_i(\lambda,q) \paren{\frac{1}{q^{i}}-\frac{1}{q^{i+1}}},\\
    P_\lambda(\qLL)=&1/q^{\max \{ i \mid Y_i(\lambda,q)=1\}+1}.
\end{align*}
\end{definition}

\subsubsection{Asymptotic Approximation}
So far, so good. Now suppose we want to calculate the expected changing probability after $\lambda$ insertions to a $\qPCSA$ sketch. We have
\begin{align*}
    \E\paren{P_\lambda(\qPCSA)} =& \sum_{i=0}^\infty (\frac{1}{q^i}-\frac{1}{q^{i+1}})\Pr(Y_i(\lambda,q)=0)\\
    =&\sum_{i=0}^\infty (\frac{1}{q^i}-\frac{1}{q^{i+1}})(1-(\frac{1}{q^i}-\frac{1}{q^{i+1}}))^\lambda= \sum_{i=0}^\infty \frac{1}{q^i}\frac{q-1}{q}(1-\frac{1}{q^i}\frac{q-1}{q})^\lambda,
\end{align*}
which is complicated to evaluate. As it is done in \cite{PettieW20}, since we care the asymptotic behavior of the sketches as $\lambda \to \infty$, we do the following assumptions and simplifications to the base-$q$ quantization.
\begin{enumerate}
    \item The probability that $Y_i(\lambda,q)$ is zero is equal to \emph{exactly} 
    $ e^{-\lambda (\frac{1}{q^i}-\frac{1}{q^{i+1}})}$.
    \item The random variables $(Y_i(\lambda,q))_{i\geq 0}$ are independent.
    \item We extend the domain of the sketch $\mathbf{b}$ from $\mathbb{N}$ to $\mathbb{Z}$, e.g., together with
    assumption (1), 
    $\mathbb{P}(Y_{-5}(q,\lambda) = 0) = e^{-\lambda (q^5-q^4)}$.
\end{enumerate}

\subsubsection{Smoothing Technique (Offsetting)}
Applying the asymptotic approximation, now we have
\begin{align}\label{eq:asymp_ep}
    \E\paren{P_\lambda(\qPCSA)} = \sum_{i=-\infty}^\infty \frac{1}{q^i}\frac{q-1}{q} e^{-\frac{\lambda}{q^i}\frac{q-1}{q}}.
\end{align}
This becomes ``weakly'' scale-invariant in the sense that
\begin{align*}
    \E\paren{P_{q\lambda}(\qPCSA)} = \sum_{i=-\infty}^\infty \frac{1}{q^i}\frac{q-1}{q} e^{-\frac{q\lambda}{q^i}\frac{q-1}{q}} = \frac{1}{q}\sum_{i=-\infty}^\infty \frac{1}{q^{i-1}}\frac{q-1}{q} e^{-\frac{\lambda}{q^{i-1}}\frac{q-1}{q}}=\frac{1}{q}\E\paren{P_{\lambda}},
\end{align*}
which says that the quantity $\lambda \E\paren{P_\lambda(\qPCSA)}$ is multiplicatively periodic with period $q$.

To make it strictly scale-invariant, we randomly ``offset'' the quantization $Y(q,\lambda)$. Specifically, let $r\in[0,1)$, we define a base-$q$ quantization with offset $r$ of $X(\lambda)$ to be a set of random variables $Y(\lambda,q,r)=\{Y_i(\lambda,q,r)\}_{i\geq 0}$ where for any $i\geq 0$,
\begin{align*}
    Y_i(\lambda,q,r)= \mathbbm{1}\left[ X(\lambda )\cap (\frac{1}{q^{i+1+r}},\frac{1}{q^{i+r}}]\neq \emptyset \right].
\end{align*}
Note that the offset technique has a simple algorithmic implementation: a sketch with base $q$ that is offset by $r$ just needs to run as usual except for only processing a new insertion with probability $q^{-r}$.

Using the asymptotic approximation, we have
\begin{align*}
    \Pr(Y_i(\lambda,q,r)=0)=e^{-\lambda(\frac{1}{q^{i+r}}-\frac{1}{q^{i+1+r}}))}.
\end{align*}


Now consider a $\qPCSA$ sketch with a random offset $R$ where $R$ is a uniform random variable in $[0,1)$. By the law of total expectation, we have (using formula (\ref{eq:asymp_ep}))
\begin{align*}
    \E(P_\lambda(\qPCSA)) =& \E\paren{\E\paren{P_\lambda(\qPCSA;r=R) \mid R}}=\int_0^1  \sum_{i=-\infty}^\infty\frac{1}{q^{i+r}}\frac{q-1}{q} e^{-\frac{\lambda}{q^{i+r}}\frac{q-1}{q}} dr\\
    =&\int_{-\infty}^\infty  \frac{1}{q^{t}}\frac{q-1}{q} e^{-\frac{\lambda}{q^{t}}\frac{q-1}{q}} dr=\int_{-\infty}^\infty  \frac{1}{q^{t}} e^{-\frac{\lambda}{q^{t}}} dr\\
    =&\frac{1}{\lambda \log q}.
\end{align*}
Finally, with a uniformly random offset, $\lambda \E(P_\lambda)=\frac{1}{\log q}$ is a constant and therefore it is scale-invariant.


\subsection{Analyzing Sketches}
\begin{theorem}
The smoothed $\qLL$ and $\qPCSA$ are scale-invariant. In particular, we have,
\begin{align*}
    \kappa_{\qLL} = \frac{1}{\log q}\frac{q-1}{q},\text{ and }\kappa_{\qPCSA}=\frac{1}{\log q}.
\end{align*}
\end{theorem}
\begin{proof}
For $\qLL$, 
\begin{align*}
\E(P_\lambda) &=\int_0^1\sum_{k=-\infty}^\infty (e^{-\frac{\lambda}{q^{k+r}}}-e^{-\frac{\lambda}{q^{k-1+r}}})\frac{1}{q^{k+r}} dr\\
    &= \int_{-\infty}^\infty (e^{-\frac{\lambda}{q^t}}-e^{-\frac{\lambda}{q^{t-1}}})\frac{1}{q^t} dt\\
    &= \frac{1}{\lambda\log q}-\frac{1}{q\lambda \log q}\\
    &= \frac{1}{\lambda\log q}\frac{q-1}{q}.
\end{align*}
Thus we have $\lambda \E(P_\lambda)=\frac{1}{\log q}\frac{q-1}{q}$.

For $\qPCSA$, as calculated previously, we have $\lambda \E(P_\lambda)=\frac{1}{\log q}$.
\end{proof}


\begin{theorem}
\begin{align*}
    &\MVP(\qPCSA,\text{perfect compression})=\frac{H_0}{2},\\
    &\MVP(\qLL, \text{perfect compression})=\frac{q}{q-1}\frac{\phi(q)}{2},
\end{align*}
where
\begin{align*}
     H_0 =& \frac{1}{\ln 2} + \sum_{k=1}^\infty\frac{1}{k}\log_2 \left(1+1/k\right),\\
     \phi(q) =& \frac{1-1/q}{\ln 2} + \sum_{k=1}^\infty\frac{1}{k}\log_2 \left(\frac{k+\frac{1}{q-1}+1}{k+\frac{1}{q-1}}\right).
\end{align*}

Furthermore,
$ \MVP(\qLL, \text{perfect compression})$ decreases as $q$ increases and $$\lim_{q\to\infty}  \MVP(\qLL, \text{perfect compression}) =\frac{H_0}{2}=\MVP(\qPCSA,\text{perfect compression}).$$
\end{theorem}


It remains open whether $H_0/2$ is the optimal $\MVP$ for the class of scale-invariant sketches.

\section{New Algorithms}
The martingale estimator is flexible, in the sense that no matter what sketch one comes up with, as long as it is not affected by duplicates, one can use martingale estimator to estimate the cardinality for it, which is unbiased and has optimal variance. Thus now one can design more complicated sketches without worrying about its estimation methods. In addition, Theorem \ref{thm:kappa} provides a systematic way to compute the relative streaming variance of any scale-invariant sketch. In this section, we will explore new sketches.

\subsection{Curtain}
Consider the class of algorithms that based on a set of independent sketches. We want a counting algorithm that works for arbitrarily large $\lambda$. It is natural to store an offset that depends on $\lambda$ and the ``differences'' between sketches that don't depend on the size of $\lambda$.

For example, consider a set of $m$ HLL sketches with heights $(h_1,h_2,\ldots,h_m)$. One can store the heights in the vector $(h_1,h_2-h_1,h_3-h_2,\ldots,h_m-h_{m-1})$. Let $d_k=h_{k+1}-h_k$. Say we want to store every $d_k$ by a fixed number of bits and thus only a finite set of the possible values of $d_k$ can be encoded. In addition, we don't want to ``ruin'' any sketch. For any $k$, the difference $d_k$ could be any integer. Thus there will be cases where $d_k$ is not representable by the assigned bits. A natural way to resolve this is to ``minimally'' adjust the values of $h_i$s near $h_k$ until all the differences can be represented. 

Using Ting's martingale estimator, this ``curtain drawing'' process (since whenever you raise a single sketch, you may need to adjust its neighbours) can also be used to estimate the cardinality. 

The variance will increase by some amount, since the remaining area contracts faster than the original HLL. However, now we can safely use a fixed amount of memory to store the $d_k$s for arbitrary $\lambda$. (a diagram here to show how curtain HLL differs from original HLL)

\subsection{Sawtooth Offsetting}
Consider offsets $(0,-1/2,0,-1/2,\ldots)$. A state $(s_1,s_2,\ldots)$ is encoded by  $(s_2-s_1,s_3-s_2+1,s_4-s_3,s_5-s_4+1,\ldots)$. Let $a\in\mathbb{N}_+$ be a parameter. One requires each entry of the encoding lie in the range $(-a,a]$, which requires $\log_2 (2a)$ bits. 

\subsection{Curtain PCSA}
In this subsection we introduce a parametrized curtain algorithm based on PCSA, which covers lots of other natural curtain algorithms as subcases.

The parameters are the base $q$, the curtain limit $a$ and the number of bits explicitly stored $h$. Use curtain HLL to store the profile and store the $h$ bits under the profile. If a column is being pulled, then store the highest $h$ bits.

\begin{theorem}
\begin{align*}
    \kappa = \frac{1}{\log q}\frac{q-1}{q}\frac{q^h}{\frac{2}{q^{a-\frac{1}{2}}-1}+1/q+q^{h}-q^{h-1}}
\end{align*}
\end{theorem}

\subsection{Second Curtain}
The only parameters are the curtain limit $a$ and the base $q$.
\subsubsection{variance}
Fixing the cardinality per sketch $\lambda$ and the offset $r$, consider the random variables,
\begin{enumerate}
    \item $X$, the height of the highest 1;
    \item $Y$, the height of the second highest 1.
\end{enumerate}
For $x>y$, we have
\begin{align*}
    \mathbb{P}(X=x,Y=y) &= e^{-\lambda(\frac{1}{q^{y+1+r}}-(\frac{1}{q^{x+r}}-\frac{1}{q^{x+1+r}}))}(1-e^{-\lambda(\frac{1}{q^{x+r}}-\frac{1}{q^{x+1+r}})})(1-e^{-\lambda(\frac{1}{q^{y+r}}-\frac{1}{q^{y+1+r}})})\\
    &= (e^{-\frac{\lambda}{q^{y+1+r}}}-e^{-\frac{\lambda}{q^{y+r}}})(e^{\lambda(\frac{1}{q^{x+r}}-\frac{1}{q^{x+1+r}})}-1)
\end{align*}
and
\begin{align*}
    \mathbb{P}(X=x,Y\leq y) &=\sum_{i=-\infty}^y\mathbb{P}(X=x,Y=y)\\
    &= e^{-\frac{\lambda}{q^{y+1+r}}}(e^{\lambda(\frac{1}{q^{x+r}}-\frac{1}{q^{x+1+r}})}-1)
\end{align*}
Thus we have
\begin{align*}
     \mathbb{P}(X>y\geq Y) &=\sum_{x=y+1}^\infty \mathbb{P}(X=x,Y\leq y)\\
     &= e^{-\frac{\lambda}{q^{y+1+r}}}\sum_{x=y+1}^\infty(e^{\lambda(\frac{1}{q^{x+r}}-\frac{1}{q^{x+1+r}})}-1)
\end{align*}
and
\begin{align*}
    \mathbb{P}(X>k> Y) &= \sum_{x=k+2}^\infty \mathbb{P}(X=x,Y\leq k-1)\\
     &= e^{-\frac{\lambda}{q^{k+r}}}\sum_{x=k+1}^\infty(e^{\lambda(\frac{1}{q^{x+r}}-\frac{1}{q^{x+1+r}})}-1)
\end{align*}
and 
\begin{align*}
     \mathbb{P}(Y\leq y) &= \mathbb{P}(X\leq y) + \mathbb{P}(X>y\geq Y)\\
     &= e^{-\frac{\lambda}{q^{y+1+r}}}+e^{-\frac{\lambda}{q^{y+1+r}}}\sum_{x=y+1}^\infty(e^{\lambda(\frac{1}{q^{x+r}}-\frac{1}{q^{x+1+r}})}-1)
\end{align*}
which we define as $\phi(y+r)$. We then have
\begin{align*}
    \mathbb{P}(Y=y) &= \mathbb{P}(Y\leq y)-\mathbb{P}(Y\leq y-1)\\
    &=  (e^{-\frac{\lambda}{q^{y+1+r}}}-e^{-\frac{\lambda}{q^{y+r}}})\sum_{x=y+1}^\infty(e^{\lambda(\frac{1}{q^{x+r}}-\frac{1}{q^{x+1+r}})}-1)
\end{align*}

For a block with height $k$, it remains in the remaining area if and only if the following two independent events occur
\begin{enumerate}
    \item event $E_1$, $k$ is unoccupied and it is between the second highest bit and the first highest bit or it is above the first highest bit;
    \item event $E_2$, $k$ is above the tension point.
\end{enumerate}

\begin{align*}
    \mathbb{P}(E_1) &= \mathbb{P}(X<k)+\mathbb{P}(Y<k<X)\\
    &= e^{-\frac{\lambda}{q^{k+r}}}+e^{-\frac{\lambda}{q^{k+r}}}\sum_{x=k+1}^\infty(e^{\lambda(\frac{1}{q^{x+r}}-\frac{1}{q^{x+1+r}})}-1)
\end{align*}
\begin{align*}
    \mathbb{P}(E_2) &= \prod_{i=1}^\infty \phi(i(a-\frac{1}{2})+k+r-1)^2
\end{align*}

Thus the expected remaining area can be expressed by
\begin{align*}
    \int_0^1 \sum_{k=-\infty}^\infty \frac{1}{q^{k+r}}\frac{q-1}{q}\mathbb{P}(E_1)\mathbb{P}(E_2) dr
\end{align*}

Let $\rho(t;q)=\sum_{i=0}^\infty (e^{t\frac{q-1}{q}\frac{1}{q^i}}-1)$ and we have
\begin{align*}
    \phi(y+r)=e^{-\frac{\lambda}{q^{y+1+r}}}(1+\rho(\frac{\lambda}{q^{y+1+r}};q))
\end{align*}

Thus we have
\begin{align*}
    \mathbb{P}(E_1) &= e^{-\frac{\lambda}{q^{k+r}}}(1+\rho(\frac{\lambda}{q^{k+1+r}};q))
\end{align*}
and 
\begin{align*}
    \mathbb{P}(E_2) &= e^{-\frac{2\lambda}{q^{k+r}}\sum_{i=1}^\infty\frac{1}{q^{i(a-\frac{1}{2})}}}\prod_{i=1}^\infty (1+\rho(\frac{\lambda}{q^{k+r+i(a-\frac{1}{2})}};q))^2\\
    &= e^{-\frac{2\lambda}{q^{k+r}}\frac{1}{q^{a-\frac{1}{2}}-1}}\prod_{i=1}^\infty (1+\rho(\frac{\lambda}{q^{k+r+i(a-\frac{1}{2})}};q))^2\\
\end{align*}

Thus the remaining area is (let $t=k+r$ and $w=\frac{\lambda}{q^t}$)
\begin{align*}
    &\int_{-\infty}^\infty \frac{1}{q^t}\frac{q-1}{q}e^{-\frac{\lambda}{q^t}\frac{q^{a-\frac{1}{2}}+1}{q^{a-\frac{1}{2}}-1}}  (1+\rho(\frac{\lambda}{q^{t+1}};q))\prod_{i=1}^\infty (1+\rho(\frac{\lambda}{q^{t+i(a-\frac{1}{2})}};q))^2 dt\\
    &= \frac{1}{\lambda \log q} \frac{q-1}{q} \int_0^\infty e^{-w\frac{q^{a-\frac{1}{2}}+1}{q^{a-\frac{1}{2}}-1}}(1+\rho(\frac{w}{q};q))\prod_{i=1}^\infty (1+\rho(\frac{w}{q^{i(a-\frac{1}{2})}};q))^2 dw
\end{align*}

\subsubsection{expected space}
For a block with height $k$, we say it ``contributes'' to the space if it is above the tension point and the second highest bit and below or equal to the first highest bit. The case where the tension point is above or equal to the second highest bit contributes one more bit. Let the tension point be $T$.

Thus the expected contribution of the block with height $k$ is equal to
\begin{align*}
    \mathbb{P}(Y<k\leq X)\mathbb{P}(E_2)
\end{align*}

and thus the expected space used for a single sketch is
\begin{align*}
    \log_2(2a)+\int_0^1\left(\mathbb{P}(T\geq Y)+\sum_{k=-\infty}^\infty \mathbb{P}(Y<k\leq X)\mathbb{P}(E_2)\right)dr.
\end{align*}
Note that $\mathbb{P}(T<k)=\mathbb{P}(E_2)$.

We have
\begin{align*}
    \mathbb{P}(T\geq Y) &= \sum_{k=-\infty}^\infty \mathbb{P}(Y=k)\mathbb{P}(T\geq k)\\
    &= \sum_{k=-\infty}^\infty \mathbb{P}(Y=k)(1-\mathbb{P}(E_2))\\
    &= 1- \sum_{k=-\infty}^\infty \mathbb{P}(Y=k)\mathbb{P}(E_2)
\end{align*}
where $\mathbb{P}(Y=k)=(e^{-\frac{\lambda}{q^{k+1+r}}}-e^{-\frac{\lambda}{q^{k+r}}})\rho(\frac{\lambda}{q^{k+1+r}};q)$.

Also we have
\begin{align*}
    \mathbb{P}(Y<k\leq X) &= \sum_{x=k}^\infty \mathbb{P}(X=x,Y\leq k-1)\\
    &= e^{-\frac{\lambda}{q^{k+r}}} \sum_{x=k}^\infty (e^{\lambda(\frac{1}{q^{x+r}}-\frac{1}{q^{x+1+r}})}-1)\\
    &= e^{-\frac{\lambda}{q^{k+r}}}\rho(\frac{\lambda}{q^{k+r}};q).
\end{align*}

Thus 
\begin{align*}
    &\int_0^1\left(\mathbb{P}(T\geq Y)+\sum_{k=-\infty}^\infty \mathbb{P}(Y<k\leq X)\mathbb{P}(E_2)\right)dr\\
    &= \int_0^1\left(1+\sum_{k=-\infty}^\infty( \mathbb{P}(Y<k\leq X)-\mathbb{P}(Y=k))\mathbb{P}(E_2)\right)dr\\
    &= 1+\int_{-\infty}^\infty (e^{-\frac{\lambda}{q^t}}\rho(\frac{\lambda}{q^{t}};q)-(e^{-\frac{\lambda}{q^{t+1}}}-e^{-\frac{\lambda}{q^{t}}})\rho(\frac{\lambda}{q^{t+1}};q))e^{-\frac{2\lambda}{q^{t}}\frac{1}{q^{a-\frac{1}{2}}-1}}\prod_{i=1}^\infty (1+\rho(\frac{\lambda}{q^{t+i(a-\frac{1}{2})}};q))^2 dt\\
     &= 1+\frac{1}{\log q}\int_{0}^\infty \frac{1}{w} (e^{-w}\rho(w;q)-(e^{-\frac{w}{q}}-e^{-w})\rho(\frac{w}{q};q))e^{-2w\frac{1}{q^{a-\frac{1}{2}}-1}}\prod_{i=1}^\infty (1+\rho(\frac{w}{q^{i(a-\frac{1}{2})}};q))^2 dw
\end{align*}


